Measurements of long-range azimuthal anisotropies and associated Fourier coefficients for $pp$ collisions at $\sqrt{s}=5.02$ and $13$ TeV and $p$+Pb collisions at $\sqrt{s_{\mathrm{NN}}}=5.02$ TeV with the ATLAS detector

ATLAS measurements of two-particle correlations are presented for $\sqrt{s} = 5.02$ and $13$ TeV $pp$ collisions and for $\sqrt{s_{\mathrm{NN}}} = 5.02$ TeV $p$+Pb collisions at the LHC. The correlation functions are measured as a function of relative azimuthal angle $\Delta \phi$, and pseudorapidity separation $\Delta \eta$, using charged particles detected within the pseudorapidity interval $|\eta|{<}2.5$. Azimuthal modulation in the long-range component of the correlation function, with $|\Delta\eta|{>}2$, is studied using a template fitting procedure to remove a "back-to-back" contribution to the correlation function that primarily arises from hard-scattering processes. In addition to the elliptic, $\cos{(2\Delta\phi)}$, modulation observed in a previous measurement, the $pp$ correlation functions exhibit significant $\cos{(3\Delta\phi)}$ and $\cos{(4\Delta\phi)}$ modulation. The Fourier coefficients $v_{n,n}$ associated with the $\cos{(n\Delta\phi)}$ modulation of the correlation functions for $n =$ $2$-$4$ are measured as a function of charged-particle multiplicity and charged-particle transverse momentum. The Fourier coefficients are observed to be compatible with $\cos{(n\phi)}$ modulation of per-event single-particle azimuthal angle distributions. The single-particle Fourier coefficients $v_n$ are measured as a function of charged-particle multiplicity, and charged-particle transverse momentum for $n {=} $ $2$-$4$. The integrated luminosities used in this analysis are, $64$ $\mathrm{nb^{-1}}$ for the $\sqrt{s}=13$ TeV $pp$ data, $170$ $\mathrm{nb^{-1}}$ for the $\sqrt{s}=5.02$ TeV $pp$ data and $28$ $\mathrm{nb^{-1}}$ for the $\sqrt{s_{\mathrm{NN}}}=5.02$ TeV $p$+Pb data.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 06-Mar-2017

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DSM/IRFU, France; SRNSF, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, ERDF, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; CERCA Programme Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------


